Boosting New Physics Searches in $t\bar{t}Z$ and $tZj$ Production with Angular Moments

The angular moments for the $Z$ boson can be used as analyzers for the underlying production dynamics for the $t\bar t Z$ and $t Zj$ processes. In this manuscript, we derive these angular moments at leading and next-to-leading order in QCD at the LHC. We show that these observables work as efficient probes to beyond the Standard Model effects, considering the Standard Model Effective Field theory framework. Remarkably, we observe that these probes unveil blind directions to CP-odd operators, providing sizable new physics sensitivity at the 14 TeV LHC with 3 ab$^{-1}$ of data.

==> babelbst.tex <==
%%
%% This is file `merlin.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from merlin.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2011 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2011/11/18 4.33 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}                \def\bbletal{et~al.}
\def\bbleditors{editors}        \def\bbleds{eds.}
\def\bbleditor{editor}          \def\bbled{ed.}
\def\bbledby{edited by}
\def\bbledition{edition}        \def\bbledn{edn.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{of}
\def\bblnumber{number}          \def\bblno{no.}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapter}        \def\bblchap{chap.}
\def\bbltechreport{Technical Report}
\def\bbltechrep{Tech. Rep.}
\def\bblmthesis{Master's thesis}
\def\bblphdthesis{Ph.D. thesis}
\def\bblfirst{First}            \def\bblfirsto{1st}
\def\bblsecond{Second}          \def\bblsecondo{2nd}
\def\bblthird{Third}            \def\bblthirdo{3rd}
\def\bblfourth{Fourth}          \def\bblfourtho{4th}
\def\bblfifth{Fifth}            \def\bblfiftho{5th}
\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}
\def\bblth{th}
\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}
\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}
\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}
\endinput
%%
%% End of file `merlin.tex'.


==> header.tex <==
% Imports
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[british]{babel}

\usepackage{comment}

\usepackage{color,xcolor}
\definecolor{dark-red}{rgb}{0.8, 0.0, 0.1803921568627451}
\definecolor{dark-blue}{rgb}{0.0, 0.0, 0.803921568627451}
\definecolor{dark-green}{rgb}{0.0, 0.39215686274509803, 0.0}
\definecolor{dark-orange}{rgb}{0.8, 0.4, 0.0}

% Packages
\usepackage{amsmath,dsfont,mathtools}
\usepackage{siunitx}
\usepackage{graphicx}
\usepackage{multirow,booktabs,tabularx,float}
\usepackage{slashed,braket}
\usepackage{feynmp-auto}
\usepackage[sort&compress]{natbib}
\PassOptionsToPackage{hyphens}{url}\usepackage[colorlinks=true, urlcolor=dark-blue, anchorcolor=dark-blue, citecolor=dark-blue, filecolor=dark-blue, linkcolor=dark-blue, menucolor=dark-blue,  linktocpage=true, pdfa=true, linktoc=all]{hyperref}
\usepackage{enumitem} % for user-defined bullets
\usepackage[stretch=15,shrink=15]{microtype} % Default settings: protrusion=true,factor=1000,expansion=true,auto=true,stretch=20,shrink=20
\usepackage{tabto}
\usepackage{accents} % for \hhat
\usepackage{tikz}
\usepackage{xspace} % spaces in commands
\usetikzlibrary{arrows, decorations.markings, arrows.meta}
% \usepackage{mparhack} % avoids marginpars appearing on the wrong side, remove for final version
\usepackage{pythonhighlight} % python code snippets

% Don't open thumbnails automatically
\hypersetup{pdfpagemode=UseNone}

\makeatletter
\def\l@subsubsection#1#2{}
\makeatother

% booktabs fix for revtex
\AtBeginDocument{
  \heavyrulewidth=.08em
  \lightrulewidth=.05em
  \cmidrulewidth=.03em
  \belowrulesep=.65ex
  \belowbottomsep=0pt
  \aboverulesep=.4ex
  \abovetopsep=0pt
  \cmidrulesep=\doublerulesep
  \cmidrulekern=.5em
  \defaultaddspace= .5em
  \setlength{\tabcolsep}{0.5em}
}

% Tools

\newcommand{\fasernu}{FASER$\nu$~}
\newcommand{\toolfont}[1]{\texttt{#1}}

% Better bullet points with enumitem
\setlist[itemize]{itemsep=1pt,parsep=1pt, topsep=1pt}
\setlist[description]{leftmargin=0.4cm}

% General typesetting
\newcommand{\newparagraph}{\par\nopagebreak\bigskip\nopagebreak\noindent}
\newcommand{\arxivlink}[1]{\href{http://arxiv.org/abs/#1}{\texttt{arXiv:#1}}}
% \newcommand{\comment}[1]{\marginpar{\sffamily\scriptsize\textcolor{dark-red}{#1}}}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}

% Yes no maybe
\newcommand{\yep}{\ensuremath{\color{dark-green}{  \checkmark}}}
\newcommand{\kindof}{\ensuremath{\color{dark-blue}{  \ast}}}
\newcommand{\nope}{\ensuremath{\color{dark-red}{  \times}}}

% Spaces
\newcommand{\qqquad}{\qquad \qquad}
\newcommand{\qqqquad}{\qqquad \qqquad}
\newcommand{\qqqqquad}{\qqqquad \qqqquad}

% Physics symbols
\newcommand{\mat}[1]{\mathcal{M}_\text{#1}}
\newcommand{\ope}[1]{\mathcal{O}_{#1}}
\newcommand{\lgr}[1]{\mathcal{L}_\text{#1}}
\newcommand{\ord}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\br}{\mathrm{BR}}
\newcommand{\mpt}{{\ensuremath{\mathbf{p}_T^{\text{miss}}}}}
\newcommand{\met}{{\ensuremath{E_T^{\text{miss}}}}}
\newcommand{\phisq}{\phi^\dagger \phi}
\newcommand{\seff}{S_{\text{eff}}}

% Units
\newcommand{\cm}{\si{cm}}
\newcommand{\m}{\si{m}}
\newcommand{\um}{\si{\mu m}}
\newcommand{\ev}{\si{eV}}
\newcommand{\kev}{\si{keV}}
\newcommand{\mev}{\si{MeV}}
\newcommand{\gev}{\si{GeV}}
\newcommand{\tev}{\si{TeV}}
\newcommand{\ab}{\si{ab}}
\newcommand{\iab}{\si{ab^{-1}}}
\newcommand{\fb}{\si{fb}}
\newcommand{\ifb}{\si{fb^{-1}}}
\newcommand{\pb}{\si{pb}}
\newcommand{\ipb}{\si{pb^{-1}}}

% Distributions
\newcommand{\normal}[2]{\mathcal{N}\!\!\left(#1 \middle| #2 \right)}

% Derivatives and commutators
\newcommand{\pder}[2]{\frac {\partial #1} {\partial #2}}
\newcommand{\tder}[2]{\frac {\diff #1} {\diff #2}}
\newcommand{\ttder}[2]{\frac {\diff^2 #1} {\diff {#2}^2}}
\newcommand{\fder}[2]{\frac {\delta #1} {\delta #2}}

%Refering to Tables/Figures ...
\newcommand{\equref}[1]{Eq.\;\eqref{eq:#1}}
\newcommand{\eqsref}[2]{Eqs.\;\eqref{eq:#1} and \eqref{eq:#2}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and \ref{sec:#2}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and \ref{fig:#2}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\tablesref}[2]{Tables~\ref{table:#1} and \ref{table:#2}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{sec:#1} and \ref{sec:#2}}

% Vectors and matrices
\newcommand{\twovec}[2]{\begin{pmatrix*}[c] #1 \\ #2 \end{pmatrix*}}
\newcommand{\threevec}[3]{\begin{pmatrix*}[c] #1 \\ #2 \\ #3\end{pmatrix*}}
\newcommand{\fourvec}[4]{\begin{pmatrix*}[c] #1 \\ #2 \\ #3 \\ #4 \end{pmatrix*}}
\newcommand{\fourvecr}[4]{\begin{pmatrix*}[r] #1 \\ #2 \\ #3 \\ #4 \end{pmatrix*}}

\newcommand{\twomat}[4]{\begin{pmatrix*}[c] #1 & #2\\ #3 & #4 \end{pmatrix*}}
\newcommand{\threemat}[9]{\begin{pmatrix*}[c] #1 & #2 & #3\\ #4 & #5 & #6 \\ #7 & #8 & #9\end{pmatrix*}}
\newcommand{\twomatr}[4]{\begin{pmatrix*}[r] #1 & #2\\ #3 & #4 \end{pmatrix*}}
\newcommand{\threematr}[9]{\begin{pmatrix*}[r] #1 & #2 & #3\\ #4 & #5 & #6 \\ #7 & #8 & #9\end{pmatrix*}}

%Equations
\newcommand{\be}{\begin{equation}\begin{aligned}}
\newcommand{\ee}{\end{aligned}\end{equation}}

%Comments by Users
\newcommand{\Dorival}[1]{\textcolor{red}{[DG: #1]}}
\newcommand{\Roshan}[1]{\textcolor{blue}{[RA: #1]}}

%Changed Comment
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

%Reference style
\bibliographystyle{utphys}



